FedVS: Straggler-Resilient and Privacy-Preserving Vertical Federated Learning for Split Models

In a vertical federated learning (VFL) system consisting of a central server and many distributed clients, the training data are vertically partitioned such that different features are privately stored on different clients. The problem of split VFL is to train a model split between the server and the clients. This paper aims to address two major challenges in split VFL: 1) performance degradation due to straggling clients during training; and 2) data and model privacy leakage from clients' uploaded data embeddings. We propose FedVS to simultaneously address these two challenges. The key idea of FedVS is to design secret sharing schemes for the local data and models, such that information-theoretical privacy against colluding clients and curious server is guaranteed, and the aggregation of all clients' embeddings is reconstructed losslessly, via decrypting computation shares from the non-straggling clients. Extensive experiments on various types of VFL datasets (including tabular, CV, and multi-view) demonstrate the universal advantages of FedVS in straggler mitigation and privacy protection over baseline protocols.

==> intro.tex <==
\section{Introduction}



Federated learning (FL) ~\cite{ZHANG2021106775} is a machine learning setting where multiple devices or organizations can collaborate to train a machine learning model, while keeping the raw data decentralized without being moved to a single server or data center. Each client holds a local model which is stored locally or transferred by a server. A server can cooperate clients to transmit data and finish the training process. Horizontal FL is a common solution for those features of data overlap a lot but identifications overlap little. FedAvg~\cite{mcmahan2017communication} is a classical protocol applied in horizontal FL composed of heterogeneous devices. Compared with horizontal FL, Vertical FL (VFL) considers a setting that each client have different features of same identifications. Many new frameworks have been proposed to construct a model in VFL setting, which can be divided into two types, one is that each client has a complete model for training, such as Logistic regression for VFL~\cite{DBLP:journals/corr/abs-1911-09824}, MMVFL~\cite{DBLP:journals/corr/abs-2001-11154}. Another type is split training model, which splits a whole model to multiple clients and a server. Some protocols based on it, such as PyVertical~\cite{DBLP:journals/corr/abs-2104-00489} and SpliNN~\cite{DBLP:journals/corr/abs-1812-00564}, show its efficiency and security. Split learning is more popular and efficient in VFL, because the network structure fully utilizes heterogeneous feature from different cooperators.

%As the storage and computational capabilities of distributed devices grow, FL is a promising way to enhance the ML models' efficiency and alleviate the resource limitation. 

 %However, some challenges still remain in FL, one is system (device) heterogeneity due to existence of dropout nodes, which will slow down the model training and lead to lower convergence rate and accuracy\cite{luo2021feature}\cite{DBLP:journals/corr/abs-2012-14453}. FedAvg just ignore the result of dropout nodes. But it has little impact on the training only when the data is homogeneous across devices. FLANP~\cite{DBLP:journals/corr/abs-2012-14453} is designed for straggler-resilient FL, which utilizes faster nodes at first and includes slower nodes later. CodedPaddedFL~\cite{DBLP:journals/corr/abs-2112-08909} is another algorithm using coding theory which introduces redundancy to the data to mitigate the dropout problem. Another major challenge is privacy leakage, due to that the adversary can reconstruct the input data from transmitted raw embedding computed by clients~\cite{DBLP:journals/corr/abs-2012-02670}. In SplitFed~\cite{DBLP:journals/corr/abs-2004-12088}, differential privacy is applied for adding a noise layer on raw embedding to protect data privacy. Another protocol SFA~\cite{https://doi.org/10.48550/arxiv.2207.00165} designs a sercure aggregation method based on homomorphic encription to mask the raw embedding in split VFL. Nevertheless, these work just consider dropout problem or privacy threat. Although some horizontal FL framework, like CodedSecAgg ~\cite{DBLP:journals/corr/abs-2112-08909}, combines secure aggregation and coding method to solve both problems, there are no work in VFL research on dropout nodes at the same time protecting data privacy.
 
 A typical training process of split VFL is composed of clients' forward propagation, server's aggregation and computation, backward propagation and the update of local and global models. First, all clients forward propagate the local data using local models. Then clients transmit their embeddings (forward output) to the server. The server aggregates these embeddings for subsequent processing by a more complex model and compute the loss by collected labels and final outputs. After the computation of gradients, the server updates the global model and the gradient of embeddings is transmitted to clients for updating the local model. An ideal training round requires all clients to update their local model synchronously. 
 
 
 
 
 If there are dropouts of some clients in a training round, the missing features of these clients and the staleness of the local model will lead to slower convergence and poor performance. To alleviate this dropout problem, VAFL~\cite{DBLP:journals/corr/abs-2007-06081}, which is an asynchronous VFL protocol, allows asynchronous submission of embeddings and model update. However, it can not provide a solution for synchronous VFL and the convergence will be affected by the variation of alive clients. Another challenge in VFL is privacy leakage. \cite{jin2021cafe} \cite{li2021survey} have investigated the vulnerability of VFL and implemented inference attack based on raw embeddings, which successfully recovers the input data. To prevent inference attack, SplitFed~\cite{DBLP:journals/corr/abs-2004-12088} and VAFL introduced differential privacy (DP) in VFL, which adds a DP noise layer on raw embeddings to provide data privacy. Another protocol SFA~\cite{https://doi.org/10.48550/arxiv.2207.00165} designed a secure aggregation method based on homomorphic encription, where raw embeddings are masked and only the aggregated embedding is revealed. These methods provide privacy for clients' data but can not solve dropout problem in a synchronous VFL setting. So, our problem is : \textit{How to design a synchronous split VFL algorithm which is dropout resilient and can provide privacy for data to prevent potential inference attack?}
 
 
To answer the above question, we propose an algorithm called Dropout-Resilient and Privacy-preserving vertical federated learning for split models (FedVS). Before introducing our algorithm, we experimentally discuss the impact of dropout clients since there is no work clearly show the variation of model performance in VFL dropout scenario. For constructing the basis of our network structure, we introduce average method for aggregation and polynomial network (PN) as clients' network. Then, we specify our algorithm, where Lagrange Coded Computing (LCC) coding is applied to split VFL. We analyze its security and provide a theoretical convergence guarantee. In addition, we experimentally show the performance of our algorithm in different dropout scenarios based on multiple datasets and compare its convergence and accuracy with DP VFL~\cite{DBLP:journals/corr/abs-2007-06081}\cite{DBLP:journals/corr/abs-2004-12088}. The experimental results show that FedVS achieves nearly same convergence and performance in no dropout scenario, while providing privacy protection. Compared with DP VFL, our algorithm has less performance loss and faster convergence rate.



\subsection{Related works}

\textbf{Dropout-resilient FL:} 

\begin{itemize}
  \item [1)]\textit{Horizontal FL:} Due to the heterogeneity of devices or organizations in FL, the assumption of non i.i.d data distribution is natural, where the dropout clients with valuable features or local models may cause low accuracy of the FL model~\cite{9411833}. Dropout-resilient aggregation combined with coding method is a strong solution to handle the dropout clients. CodedPaddedFL~\cite{DBLP:journals/corr/abs-2112-08909} borrow concepts from coded distributed computing to introduce redundancy across the network, which is leveraged during the iterative learning phase so that the server can recover the data from partial responsive clients. \cite{Liu_2022} leverages Shamir secret sharing scheme to provide dropout-resilience.
Another kind of solution is designed for providing a protocol to guarantee successful training in dropout scenario. \cite{https://doi.org/10.48550/arxiv.2206.02078},\cite{DBLP:journals/corr/abs-2012-14453} permit partial participation and prove same convergence guarantee with the full participation. However, the variation of partial participants will affect the training process and the convergence is proved based on the assumption of strong convex functions \cite{DBLP:journals/corr/abs-2012-14453}. Asynchronous aggregation and update is also a replacement for synchronous FL to handle dropout problem. FedBuffer~\cite{DBLP:journals/corr/abs-2106-06639} is an asynchronous framework combined with differential privacy(DP) to protect local model's privacy and give chance to those dropout clients for later submission. It is more efficient than synchronous FL but tolerates the performance loss. 
\item[ 2)]
\textit{Vertical FL:} To the best of our knowledge, no previous work has targeted dropout problem in VFL specifically. Asynchronous VFL is the only way which has been proposed for adapting to dropout situation in VFL. VAFL~\cite{DBLP:journals/corr/abs-2007-06081} is an asynchronous protocol for VFL, which achieves compatible model performance with synchronous VFL. However, it lacks privacy protection. \cite{DBLP:journals/corr/abs-2007-06081} also introduces DP to protect the raw data but tolerates performance loss. AFSGD-VP~\cite{9463409}, which is another asynchronous algorithm, introduces tree structure aggregation to protect data privacy. But it can not guarantee information-theoretic privacy and the aggregation will fail if some clients dropout in the second aggregation. 
\end{itemize}



\textbf{Privacy-preserving FL:} To provide privacy protection in FL, there are three common methods, which are homomorphic encryption (HE), differential privacy (DP) and secure multi-party computing (MPC)~\cite{https://doi.org/10.48550/arxiv.2203.17005}. HE method is usually applied to encrypting the local updates waiting for transmitting to the server~\cite{254465}. It allows specific computation directly on the ciphertexts and is noise-free to the whole computation. However, it is inevitable to introduce significant overhead of communication and computation in FL. Compared with HE, DP is more efficient to provide privacy by injecting noise to the private data~\cite{DBLP:journals/corr/abs-2004-12088}. Nevertheless, the performance and the convergence rate of the model will be affected by the magnitude of the noise. Shamir secret sharing based MPC~\cite{kanagavelu2020two} utilizes special computation protocol to allow different clients secret share their data to the server and only the summation of the data is revealed. The advantage is that it guarantees information-theoretic privacy for shared data at the same time providing certain level of drop-out resilience. Compared to these work, FedVS further considers the dropout problem in VFL and adopt coding method to mask clients' data and model for privacy protection.







